Revocable Cryptography from Learning with Errors

Quantum cryptography leverages many unique features of quantum information in order to construct cryptographic primitives that are oftentimes impossible classically. In this work, we build on the no-cloning principle of quantum mechanics and design cryptographic schemes with key-revocation capabilities. We consider schemes where secret keys are represented as quantum states with the guarantee that, once the secret key is successfully revoked from a user, they no longer have the ability to perform the same functionality as before. We define and construct several fundamental cryptographic primitives with key-revocation capabilities, namely pseudorandom functions, secret-key and public-key encryption, and even fully homomorphic encryption, assuming the quantum subexponential hardness of the learning with errors problem. Central to all our constructions is our approach for making the Dual-Regev encryption scheme (Gentry, Peikert and Vaikuntanathan, STOC 2008) revocable.

==> applications.tex <==
\section{Applications}
\pnote{do we get anything new?}

\subsection{Ciphertext-Revocable Fully Homomorphic Encryption: Private-Key Setting}
\pnote{Should we call this tokenized fully homomorphic encryption since it is quite different from the certified deletion schemes?\\

\noindent Does the construction give malicious evaluation from LWE? check with Poremba paper and James paper and see if we have any benefits?\\


\noindent One potential benefit: in the previous papers (Por22 and BK22), homomorphically evaluated ciphertexts cannot be classically recovered.. however in the private-key setting, they can be recovered. \\

\noindent Scheme template: 
\begin{itemize}
    \item Ciphertext = dual-Regev key, regular FHE ciphertext,
    \item Key = Encryption of the FHE key under a dual-Regev ciphertext
\end{itemize}
\ \\
\noindent Highlight the fact that we only need classical fully homomorphic evaluation + relatively few qubits..\\

\noindent Drawbacks:
\begin{itemize}
    \item Private-key setting: on the positive side, only the dual-Regev part requires the private-key setting, can we define the scheme in such a way this is not an issue? 
    \item One-time security: it only guarantees security if the adversary gets to see one ciphertext (recall that it is the private-key setting)
\end{itemize}
}

\subsection{Ciphertext-Revocable Attribute-Based Encryption: Private-Key Setting} 
\pnote{is this useful at all? do we get anything interesting?}

\subsection{Calculations}

\begin{comment}
Fact: $\frac{1}{|R|}\sum_r |\alpha_{x,r}|^2 = \frac{1}{q} + \eps_x$\\

\noindent Fact: $\frac{1}{|R|}\left(\sum_r |\alpha_{x,r}|^2 + \sum_{u \neq \langle x,r \rangle} |\beta_{x,r,u}|^2 \right) = 1$. 
Thus, we have the following:
$$\min_{u} \left( \frac{1}{|R|} \left( \sum_{r} |\beta_{x,r,u}|^2 \right)\right) \leq \frac{1}{q(q-1)}\left(1 - \left(\frac{1}{q} + \eps_x \right) \right) = \frac{1}{q} - \frac{\eps_x}{q-1} $$

The quantity we wanted to bound is the following: \pnote{technically, we should look at real and imaginary parts but the following inequalities hold for both} 
\begin{eqnarray*}
& & \omega_{q}^{\langle x,r \rangle} \left( \frac{1}{|R|} \sum_{r} |\alpha_{x,r}|^2 \right) + \sum_{u \neq \langle x,r \rangle} \omega_{q}^{u} \left( \frac{1}{|R|} \sum_{r} |\beta_{x,r,u}|^2 \right) \\
& \geq & \omega_{q}^{\langle x,r \rangle} \left( \frac{1}{|R|} \sum_r |\alpha_{x,r}|^2 \right) + \left( \sum_{u \neq \langle x,r \rangle} \omega_{q}^{u} \right) \cdot \min_{u} \left( \frac{1}{|R|} \left( \sum_{r} |\beta_{x,r,u}|^2 \right)\right) \\ 
& = & \omega_{q}^{\langle x,r \rangle} \left( \frac{1}{|R|} \sum_r |\alpha_{x,r}|^2 \right) - \left( \omega_{q}^{\langle x,r \rangle} \right) \cdot \min_{u} \left( \frac{1}{|R|} \left( \sum_{r} |\beta_{x,r,u}|^2 \right)\right) \\
& \geq & \omega_{q}^{\langle x,r \rangle} \left( \left(\frac{1}{q} + \eps_x \right) - \left(\frac{1}{q} - \frac{\eps_x}{q-1} \right) \right) \\
& = & \omega_{q}^{\langle x,r \rangle} \left( \frac{(q)}{q-1} \cdot \eps_x \right)
\end{eqnarray*}

\paragraph{New proof.}
\end{comment}

Fact: $\frac{1}{|R|}\sum_r |\alpha_{x,r}|^2 = \frac{1}{q} + \eps_x$\\

\noindent Fact: $\frac{1}{|R|}\left(\sum_r |\alpha_{x,r}|^2 + \sum_{r \in R} \sum_{u:u \neq \langle x,r \rangle} |\beta_{x,r,u}|^2 \right) = 1$. Note that we can write the above expression as follows:
$$\frac{1}{|R|}\left(\sum_r |\alpha_{x,r}|^2 + \sum_{u_1 \in \Zq} \sum_{\substack{u_2 \in \Zq,\\u_2 \neq u_1}} \sum_{r \in R: u_1 = \langle x,r \rangle} |\beta_{x,r,u}|^2 \right) = 1$$
Thus, we have the following:
$$\min_{u} \left( \frac{1}{|R|} \left( \sum_{r \in R: u = \langle x,r \rangle} |\beta_{x,r,u}|^2 \right)\right) \leq \frac{1}{q(q-1)}\left(1 - \left(\frac{1}{q} + \eps_x \right) \right) = \frac{1}{q^2} - \frac{\eps_x}{q(q-1)} $$
\pnote{NEW!!} We also have the following:
$$\max_{u} \left( \frac{1}{|R|} \left( \sum_{r \in R: u = \langle x,r \rangle} |\beta_{x,r,u}|^2 \right)\right) \geq \frac{1}{q(q-1)}\left(1 - \left(\frac{1}{q} + \eps_x \right) \right) = \frac{1}{q^2} - \frac{\eps_x}{q(q-1)} $$
The proof of the above is the following:
\begin{eqnarray*}
\frac{1}{|R|} \left( \sum_{r \in R: u = \langle x,r \rangle} |\beta_{x,r,u}|^2 \right) = 
\end{eqnarray*}


The quantity we wanted to bound is the following: \pnote{technically, we should look at real and imaginary parts but the following inequalities hold for both} 
\begin{eqnarray*}
& & \frac{1}{|R|} \sum_{r} \left(|\alpha_{x,r}|^2 \right) + \frac{1}{|R|} \sum_{r} \left( \sum_{u \neq \langle x,r \rangle} \omega_{q}^{u - \langle x,r \rangle} \left( |\beta_{x,r,u}|^2 \right) \right) \\
& = & \frac{1}{|R|} \sum_{r} \left(|\alpha_{x,r}|^2 \right) + \sum_{u_1} \sum_{u_2: u_2 \neq u_1} \omega_{q}^{u_2 - u_1} \left( \frac{1}{|R|} \sum_{r:\langle x,r \rangle = u_1} \left( |\beta_{x,r,u}|^2 \right) \right) \\
& \geq & \left( \frac{1}{|R|} \sum_r |\alpha_{x,r}|^2 \right) + \left( \sum_{u_1} \sum_{u_2:u_1 \neq u_2} \omega_{q}^{u_2 - u_1} \right) \cdot \min_{u_1} \left( \frac{1}{|R|} \left( \sum_{r \in R: u_1 = \langle x,r \rangle} |\beta_{x,r,u}|^2 \right)\right)  \\ 
& = & \left( \frac{1}{|R|} \sum_r |\alpha_{x,r}|^2 \right) + \left( \sum_{u_1} (-1) \right) \cdot \min_{u_1} \left( \frac{1}{|R|} \left( \sum_{r} |\beta_{x,r,u}|^2 \right)\right) \\
& = &\left( \left(\frac{1}{q} + \eps_x \right) + (-q) \cdot \left( \min_{u_1} \left( \frac{1}{|R|} \left( \sum_{r:\langle x,r \rangle = u_1} |\beta_{x,r,u}|^2 \right)\right) \right) \right) \\
& \geq & \frac{1}{q} + \eps_x - \frac{1}{q} + \frac{\eps_x}{(q-1)} \\
& = & \frac{q \eps_x}{q-1}
%& = & \omega_{q}^{\langle x,r \rangle} \left( \frac{(q-1)}{q} \cdot \eps \right)
\end{eqnarray*}

\noindent The success probability for a fixed $x$ is $\frac{(q \eps_x)^2}{(q-1)^2}$ Note that the success probability of the predictor is $\eps = \mathbb{E}[\eps_x]$. Thus, we have the success probability of the inverter is ?? (use Jensen's?). 

==> implications.tex <==
\section{Key-Revocable Fully Homomorphic Encryption}\label{sec:dual-GSW}

In this section, we describe our key-revocable (leveled) fully homomorphic encryption scheme from $\LWE$ which is based on the so-called $\mathsf{DualGSW}$ scheme used by Mahadev~\cite{mahadev2018classical} which itself is a variant of the homomorphic encryption scheme by Gentry, Sahai and Waters~\cite{GSW2013}.

Let $\lambda \in \N$ be the security parameter. Suppose we would like to evaluate $L$-depth circuits consisting of $\mathsf{NAND}$ gates. We choose $n(\lambda,L) \gg L$ and a prime $q=2^{o(n)}$. Let $m \geq 2 n \log q$ and $N = (n+1) \cdot \lceil \log q \rceil$, and let $\vec G \in \Z_q^{(m+1) \times N}$ denote the so-called \emph{gadget matrix} which converts a binary representation of a vector back to its original vector representation over the field $\Z_q$. More precisely, for any binary vector $\vec a = (a_{1,0},\hdots, a_{1,l-1},\hdots,a_{m+1,0},\hdots,a_{m+1,l-1})$ of length $N$ with $\ell = \lceil \log q \rceil$, the matrix $\vec G$ produces a vector in $\Z_q^{m+1}$ as follows:

\begin{align}\label{eq:matrix-G}
\vec G(\vec a) = \left(
\sum_{j=0}^{\lceil \log q \rceil-1} 2^j \cdot a_{1,j} \,\,\,, \hdots, \sum_{j=0}^{\lceil \log q \rceil-1} 2^j \cdot a_{m+1,j}
\right).
\end{align}
Note that the associated (non-linear) inverse operation $\vec G^{-1}$ converts a vector $\vec a \in \Z_q^{m+1}$ to its binary representation in $\bit^N$. In other words, we have that $\vec G^{-1} \cdot \vec G = I$ acts as the identity.


\begin{construction}[Key-Revocable \textsf{DualGSW} encryption]\label{cons:DualGSW}
Let $\lambda \in \N$ be the security parameter.
The scheme $\mathsf{RevDualGSW} = (\KeyGen,\Enc,\Dec,\Eval,\Revoke)$ consists of the following $\QPT$ algorithms:
\begin{description}
\item $\KeyGen(1^\lambda,1^L) \rightarrow (\pk,\sk):$ 
sample a pair $(\vec A \in \Z_q^{n \times m},\mathsf{td}_{\vec A}) \leftarrow \GenTrap(1^n,1^m,q)$ and generate a Gaussian superposition $(\ket{\psi_{\vec y}}, \vec y) \leftarrow \mathsf{GenGauss}(\vec A,\sigma)$ with
$$
\ket{\psi_{\vec y}} \,\,= \sum_{\substack{\vec x \in \Z_q^m\\ \vec A\vec x = \vec y}}\rho_{\sigma}(\vec x)\,\ket{\vec x},
$$
for some $\vec y \in \Z_q^n$.
Output $\pk = (\vec A,\vec y)$, $\sk = \ket{\psi_{\vec y}}$ and $\msk = \mathsf{td}_{\vec A}$.

\item $\Enc(\pk,b):$ to encrypt $b \in \bit$, parse $(\vec A,\vec y) \leftarrow \pk$, sample a random matrix $\vec S \rand \Z_q^{n \times N}$ and $\vec E \sim D_{\Z^{m\times N}, \,\alpha q}$ and row vector $\vec e \sim D_{\Z^{N}, \,\beta q}$, and
output the ciphertext 
$$
\ct= \left[\substack{
\vec A^\intercal \vec S + \vec E\vspace{1mm}\\
\hline\vspace{1mm}\\
\vec y^\intercal  \vec S + \vec e}
 \right] 
+ b \cdot \vec G \Mod{q} \in \Z_q^{(m+1)\times N}.
$$

\item $\Eval(\ct_0,\ct_1):$ to apply a $\mathsf{NAND}$ gate on a ciphertext pair $\ct_0$ and $\ct_1$, output the matrix
$$
\vec G - \ct_0 \cdot \vec G^{-1}(\ct_1) \Mod{q} \in \Z^{(m+1)\times N}.
$$


\item $\Dec(\sk,\ct) \rightarrow \bit:$ to decrypt $\ct$, 
apply the unitary $U: \ket{\vec x}\ket{0} \rightarrow \ket{\vec x}\ket{(-\vec x,1)^\intercal \cdot \ct_N}$ on input $\ket{\psi_{\vec y}}\leftarrow\sk$, where $\ct_N \in \Z_q^{m+1}$ is the $N$-th column of $\ct$, and measure the second register in the computational basis. Output $0$, if the measurement outcome
is closer to $0$ than to $\lfloor \frac{q}{2} \rfloor$,
and output $1$, otherwise.

\item $\revoke(\msk,\pk,\rho) \rightarrow \{\top,\bot\}$: on input $\mathsf{td}_{\vec A} \leftarrow \msk$ and $(\vec A,\vec y) \leftarrow \pk$, apply the projective measurement $\{\ketbra{\psi_{\vec y}}{\psi_{\vec y}},I  - \ketbra{\psi_{\vec y}}{\psi_{\vec y}}\}$ onto $\rho$ using $\mathsf{SampGauss}(\vec A,\mathsf{td}_{\vec A},\vec y,\sigma)$ in Algorithm \ref{alg:SampGauss}. Output $\top$ if the measurement is successful, and output $\bot$ otherwise.
\end{description}
\end{construction}


\begin{theorem}\label{thm:security-Dual-GSW}
Let $L$ be an upper bound on the $\mathsf{NAND}$-depth of the circuit which is to be evaluated. Let $n\in \N$ and $q$ be a prime modulus with $n=n(\lambda,L) \gg L$, $q=2^{o(n)}$ and $m \geq 2n \log q$, each parameterized by the security parameter $\lambda \in \N$. Let $N = (n+1) \cdot \lceil \log q \rceil$ be an integer. Let $\sigma \in (\sqrt{2m},q/\sqrt{2m})$ and let $\alpha,\beta \in (0,1)$ be parameters such that $\beta/\alpha =2^{o(n)}$ and $1/\alpha= 2^{o(n)} \cdot \sigma$.
Then, assuming the subexponential hardness of the $\mathsf{LWE}_{n,q,\alpha q}^m$
and $\mathsf{SIS}_{n,q,\sigma\sqrt{m}}^m$ problems, the scheme
$\mathsf{RevDualGSW} = (\KeyGen,\Enc,\Dec,\Eval,\Revoke)$ in \Cref{cons:DualGSW}
is a secure key-revocable (leveled) fully homomorphic encryption scheme according to \Cref{def:krpke:security}.
\end{theorem}

\begin{proof} Fix a $\QPT$ adversary $\algo A$. We consider the following hybrids.
\begin{description}
\item $\mathbf{H_0:}$ This is the original experiment:
\begin{enumerate}
    \item The challenger samples $(\vec A \in \Z_q^{n \times m},\mathsf{td}_{\vec A}) \leftarrow \GenTrap(1^n,1^m,q)$ and generates
$$
\ket{\psi_{\vec y}} \,\,= \sum_{\substack{\vec x \in \Z_q^m\\ \vec A \vec x = \vec y}}\rho_{\sigma}(\vec x)\,\ket{\vec x},
$$
for some $\vec y \in \Z_q^n$. The challenger assigns $\msk \leftarrow \mathsf{td}_{\vec A}$ and sends $\sk \leftarrow \ket{\psi_{\vec y}}$ to $\mathcal A$.
\item $\mathcal A$ generates a (possibly entangled) bipartite state $\rho_{R \,\vec{\textsc{aux}}}$ in systems $\algo H_R \otimes \algo H_{\textsc{aux}}$ with $\algo H_R=(\mathbb{C}^q)^{\otimes m}$, returns system $R$ and holds onto the auxiliary system $\textsc{aux}$.
\item The challenger runs $\revoke(\msk,\pk,\rho_R)$, where $\rho_R$ is the reduced state in system $R$. If successful with outcome $\top$, the experiment continues. Otherwise, $\algo A$ loses.
\item The challenger samples a random matrix $\vec S \rand \Z_q^{n \times N}$ and errors $\vec E \sim D_{\Z^{m\times N}, \,\alpha q}$ and row vector $\vec e \sim D_{\Z^{N}, \,\beta q}$, and
outputs the ciphertext 
$$
\ct
= \left[\substack{
\vec A^\intercal \vec S + \vec E\vspace{1mm}\\
\hline\vspace{1mm}\\
\vec y^\intercal  \vec S + \vec e}
 \right] 
\,\, \in \Z_q^{(m+1)\times N}.
$$
\item $\algo A$ returns a bit $b' \in \bit$, which is also the outcome of the experiment.
\end{enumerate}

\item $\mathbf{H_1:}$ This is the same as $\mathbf{H_0}$, except that instead of $\ct$, the challenger outputs 
$$
\left[\substack{
\, \vec U \, \vspace{1mm}\\
\hline\vspace{1mm}\\
\vec r}
 \right] 
\,\, \in \Z_q^{(m+1)\times N}.
$$
where $\vec U \rand \Z_q^{m \times N}$ is a random matrix and $r \rand \Z_q^N$ is a random row vector.

\item $\mathbf{H_2:}$ This is the same as $\mathbf{H_1}$, except that the challenger samples a random matrix $\vec S \rand \Z_q^{n \times N}$ and errors $\vec E \sim D_{\Z^{m\times N}, \,\alpha q}$ and column vector $\vec e \sim D_{\Z^{N}, \,\beta q}$
, and outputs the ciphertext 
$$
\ct
= \left[\substack{
\vec A^\intercal \vec S + \vec E\vspace{1mm}\\
\hline\vspace{1mm}\\
\vec y^\intercal  \vec S + \vec e}
 \right] + \vec G
\,\, \in \Z_q^{(m+1)\times N}.
$$
\end{description}
We now show that above hybrids are computationally indistinguishable.

\begin{claim} Assuming the subexponential hardness of $\mathsf{LWE}_{n,q,\alpha q}^m$
and $\mathsf{SIS}_{n,q,\sigma\sqrt{m}}^m$, we have
$$
| \Pr[\mathbf{H_0}= 1]  - \Pr[\mathbf{H_1}= 1]| \leq \negl(\lambda).
$$
\end{claim}
\begin{proof}
This follows from \Cref{thm:security-Dual-Regev} by sequentially invoking the security of our key-revocable Dual-Regev public-key encryption scheme in \Cref{cons:dual-regev}, for each column $i \in [N]$ in $\ct$.
\end{proof}

Using a similar argument, we can also prove the following:

\begin{claim} Assuming the subexponential hardness of $\mathsf{LWE}_{n,q,\alpha q}^m$
and $\mathsf{SIS}_{n,q,\sigma\sqrt{m}}^m$, we have
$$
| \Pr[\mathbf{H_1}= 1]  - \Pr[\mathbf{H_2}= 1]| \leq \negl(\lambda).
$$
\end{claim}
This concludes the proof.
\end{proof}

==> proof-distinctpreimage.tex <==

\begin{proof}
\noindent Expanding the probability, we have the following: 
\begin{eqnarray*}
& & \prob\left[(\vec x,\vec x') \leftarrow {\sf SimultExt}(1^n,1^m,{\vec A})\ |\ \vec A \rand \Zq^{n \times m}\right] \\
& = & \sum_{{\bf A} \in \Zq^{n \times m},{\vec y} \in \Zq^n} \Tr\left[ \Gamma_{{\vec A},{\vec y}}(\xi)\right] \cdot \prob\left[ \substack{{\vec A} \rand \Zq^{n \times m} \\ (\ket{\psi_{\vec y}},\vec y) \leftarrow \mathsf{GenGauss}(\vec A,\sigma)\\ \xi \leftarrow \adversary({\vec A},{\vec y},\ketbra{\psi_{{\vec y}}}{\psi_{{\vec y}}})} \right] 
\end{eqnarray*}

Consider the following claim. 


\end{proof}

==> tempfiles.tex <==
%@INPROCEEDINGS{1366257,
 % author={Micciancio, D. and Regev, O.},
  %booktitle={45th Annual IEEE Symposium on Foundations of Computer Science}, 
  %title={Worst-case to average-case reductions based on Gaussian measures}, 
  %year={2004},
  %volume={},
  %number={},
  %pages={372-381},
  %doi={10.1109/FOCS.2004.72}}
  
 %@misc{brakerski2021cryptographic,
 %     title={A Cryptographic Test of Quantumness and Certifiable Randomness from a Single Quantum Device}, 
  %    author={Zvika Brakerski and Paul Christiano and Urmila Mahadev and Umesh Vazirani and Thomas Vidick},
   %   year={2021},
    %  eprint={1804.00640},
    %  archivePrefix={arXiv},
     % primaryClass={quant-ph}
%}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{lemma}
Assuming QLWE, the following distributions are computationally indistinguishable:
\begin{itemize}
    \item $\{\bfA, \bfs \bfA + \bfe, \bfaux(\bfA,\mxtd) \}$ and, 
    \item $\{\bfA, \bfu, \bfaux(\bfA,\mxtd) \}$,
\end{itemize}
where $\bfA \xleftarrow{\$} \Zq^{n \times m}$, $\bfs \leftarrow \Zq^{1 \times n}$, $\bfe \leftarrow \chi^{1 \times m}$ and finally, $\bfaux(\bfA,\mxtd)$ is such that $H_{\infty}\left( \mxtd | \bfaux(\bfA,\mxtd) \right) \geq n$ \pnote{check!}. 
\end{lemma}
\begin{proof}[Proof Sketch]
We prove this by a hybrid argument:\\
\ \\
\noindent $\hybrid_1$: $\{\bfA, \bfs \bfA + \bfe, \bfaux(\bfA,\mxtd) \}$\\
\ \\
\noindent $\hybrid_2$: $\{{\color{blue} \bfA}, \bfs {\color{blue} \bfA} + \bfe, \bfaux(\bfA,\mxtd) \}$, where:\\
${\color{blue} \bfA} = M_1 \cdot M_2$ with $M_1 \xleftarrow{\$} \Zq^{n \times k}$, $M_2 \xleftarrow{\$} \{+1,-1\}^{k \times m}$ such that: (i) $k \gg n$ and, (ii) there exists $\mxtd$ such that $M_2 \cdot \mxtd = {\bf 0}$ (i.e., $M_2$ is not full rank).  
\par $\hybrid_1$ and $\hybrid_2$ are statistically indistinguishable from leftover hash lemma \pnote{check! there is side info here -- need a stronger statement here!! {\bf IMPORTANT}: Given ${\bf A}$ along with trapdoor ${\bf T}$, should not be able to distinguish $\hybrid_1$ versus $\hybrid_2$}. \\

\noindent $\hybrid_3$: $\{\bfA = {\color{blue} M_1 \cdot M_2},\  (\bfs {\color{blue} M_1} + \bfe) \cdot {\color{blue} M_2}, \bfaux(\bfA,\mxtd) \}$
\par $\hybrid_2$ and $\hybrid_3$ are perfectly indistinguishable \pnote{check!}. \\

\noindent $\hybrid_4$: $\{\bfA= M_1 \cdot M_2,\  {\color{blue} \bfu} \cdot M_2, \bfaux(\bfA,\mxtd) \}$,
where ${\color{blue} \bfu} \xleftarrow{\$} \Zq^{1 \times m}$. 
\par $\hybrid_3$ and $\hybrid_4$ are computationally indistinguishable from the security of QLWE. \pnote{here the fact that $\mxtd$ is computed only using $M_2$ is crucially used.}\\

\noindent $\hybrid_5$: $\{\bfA= M_1 \cdot M_2, \bfu, \bfaux(\bfA,\mxtd) \}$,
where ${\color{blue} \bfu} \xleftarrow{\$} \Zq^{1 \times m}$. 
\par \pnote{Use Goldreich-Levin to extract $M_2$ (see the pic on phone). Once $M_2$ is extracted, we can derive ${\bf T}$ and using ${\bf T}$, we can derive ${\bf T_f}$. Now we have one ${\bf T}_f$ and we can get a possibly different ${\bf T}_f$ from the state returned by the adversary. Using this, we can violate SIS for $[{\bf A}|{\bf A}_f]$.\\

Issue: we might only be able to extract one row of $M_2$. We need to do something clever to extract all the rows of $M_2$. For example, the adversary might only be distinguishing the $i^{th}$ column of ${\bf u}\cdot M_2$ and we have to trick this adversary into extracting multiple columns of $M_2$. }  
\end{proof}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

